From Patching to Pruning Visual Computation in Vision Language Models

Vision language models (VLMs) incur substantial inference cost because every visual token is processed by the attention and MLP projections of every decoder layer, even when token-specific visual computation is unnecessary at many depths. We introduce Patch-to-Prune (P2P), inspired by Mechanistic Interpretability, a training-free framework that converts activation patching from a diagnostic tool into an inference-time computation bypass. P2P performs validation-guided forward and backward layer sweeps to identify decoder regions whose visual-token projection outputs can be replaced by fixed neutral proxy activation vectors within a user-specified accuracy tolerance. Unlike conventional token-pruning methods, P2P preserves the sequence length, token order, positional information, attention mask, and residual pathways, thereby pruning computation without removing tokens or modifying the pretrained model weights. We evaluate P2P on four VLMs from the Qwen2.5-VL and LLaVA families across seven multi-modal benchmarks using mutually disjoint calibration, validation, and test partitions. P2P at a 3% tolerance retains around 94% of dense accuracy while reducing FLOPs by 55%. Beyond these efficiency gains, our layer-wise analysis suggests that visual processing in VLMs is non-uniformly distributed across decoder depth: early and late layers often require little token-specific visual computation, whereas intermediate layers appear to perform most task-relevant visual integration, enabling later reasoning to rely largely on visual information already embedded in shared residual and textual representations. This makes P2P both an efficient inference framework and a causal lens into visual information processing in VLMs.

==> tables/mainresperc.tex <==
% \begin{table*}[t]
% \centering
% \caption{Accuracy and FLOPs relative to the corresponding Dense model. Each dataset value is reported as a percentage of Dense, so Dense equals 100\%. Avg. is the arithmetic mean across available datasets. For each model and dataset, the best non-Dense accuracy and lowest non-Dense FLOPs are bolded; the same rule is applied to the Avg. column.}
% \label{tab:all_models_baselines_p2p_acc_flops_percent_dense}

% \begin{tabular}{clllccccccccc}
% \hline
%  & Method & Metric & Tol. & wco & wvg & pope & sqa & gqa & tvqa & cvb & ai2d & Avg. \\
% \hline
% \multirow{12}{*}{\rotatebox{90}{\textbf{LLaVA-v1.6-Vicuna-7B}}} & Dense & Acc. (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
%  & Dense & FLOPs (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
% \cline{2-13}
%  & FastV & Acc. (\% Dense) & -- & 97.1\% & 96.7\% & 99.2\% & 99.7\% & \textbf{99.6\%} & 99.3\% & 101.2\% & 98.7\% & 98.9\% \\
%  & FastV & FLOPs (\% Dense) & -- & 52.6\% & 52.8\% & 51.9\% & 53.4\% & 51.9\% & 52.8\% & 52.7\% & 52.6\% & 52.6\% \\
% \cline{2-13}
%  & PDrop & Acc. (\% Dense) & -- & \textbf{98.4\%} & 98.5\% & \textbf{100.1\%} & \textbf{100.5\%} & 99\% & \textbf{99.8\%} & \textbf{101.4\%} & 99\% & \textbf{99.6\%} \\
%  & PDrop & FLOPs (\% Dense) & -- & 47.3\% & 47.5\% & 46.6\% & 48\% & \textbf{46.5\%} & \textbf{47.6\%} & 47.4\% & 47.3\% & 47.3\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 1\% & 90.6\% & \textbf{109.5\%} & -- & 99.7\% & 98.6\% & 88.8\% & 93\% & 99.6\% & 97.1\% \\
%  & P2P & FLOPs (\% Dense) & 1\% & 30.7\% & 47\% & -- & 52\% & 74.5\% & 61.4\% & 30.6\% & 55.2\% & 50.2\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 3\% & 88.8\% & 98.9\% & 98\% & 96.4\% & 93.7\% & 87.3\% & 84.7\% & \textbf{99.8\%} & 93.4\% \\
%  & P2P & FLOPs (\% Dense) & 3\% & \textbf{11.3\%} & 35.9\% & 49.4\% & 32.4\% & 66.1\% & 55.9\% & 22.3\% & 52.4\% & 40.7\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 5\% & 88.8\% & 97.4\% & 91.5\% & 88\% & 90.9\% & 75.6\% & 84.4\% & 97.6\% & 89.3\% \\
%  & P2P & FLOPs (\% Dense) & 5\% & \textbf{11.3\%} & \textbf{27.6\%} & \textbf{43.8\%} & \textbf{10.1\%} & 52\% & 47.7\% & \textbf{19.5\%} & \textbf{44.1\%} & \textbf{32\%} \\
% \hline
% \multirow{12}{*}{\rotatebox{90}{\textbf{LLaVA-v1.6-Vicuna-13B}}} & Dense & Acc. (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
%  & Dense & FLOPs (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
% \cline{2-13}
%  & FastV & Acc. (\% Dense) & -- & 97.7\% & 99.2\% & 98.4\% & 99\% & 99.3\% & 98.9\% & 99.6\% & 99.8\% & 99\% \\
%  & FastV & FLOPs (\% Dense) & -- & 52.3\% & 52.5\% & 51.7\% & 53\% & 51.6\% & 52.6\% & 52.5\% & 52.4\% & 52.3\% \\
% \cline{2-13}
%  & PDrop & Acc. (\% Dense) & -- & 97.5\% & 98.9\% & \textbf{99.8\%} & 99.2\% & \textbf{100\%} & \textbf{99.8\%} & \textbf{100.1\%} & \textbf{100.1\%} & \textbf{99.4\%} \\
%  & PDrop & FLOPs (\% Dense) & -- & 47.5\% & 47.7\% & 46.8\% & 48.1\% & \textbf{46.7\%} & \textbf{47.8\%} & 47.7\% & 47.6\% & 47.5\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 1\% & \textbf{101.1\%} & \textbf{103.3\%} & 99.3\% & \textbf{99.9\%} & 91.9\% & 98.5\% & 88.7\% & -- & 97.5\% \\
%  & P2P & FLOPs (\% Dense) & 1\% & 79.6\% & 88.4\% & 45.1\% & 49.7\% & 51.8\% & 95.4\% & 23.3\% & -- & 61.9\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 3\% & 96.4\% & 100.5\% & 98.8\% & 97.9\% & 91.9\% & 90.6\% & 88.7\% & 90.7\% & 94.5\% \\
%  & P2P & FLOPs (\% Dense) & 3\% & 30.1\% & 34.3\% & 29.1\% & 40.7\% & 51.8\% & 59.6\% & 23.3\% & 31.9\% & 37.6\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 5\% & 89.5\% & 89.3\% & 92.4\% & 96.5\% & 85.2\% & 90\% & 64.8\% & 87\% & 86.8\% \\
%  & P2P & FLOPs (\% Dense) & 5\% & \textbf{25.6\%} & \textbf{29.8\%} & \textbf{24.5\%} & \textbf{29.3\%} & 47.2\% & 55.2\% & \textbf{12\%} & \textbf{27.4\%} & \textbf{31.4\%} \\
% \hline
% \multirow{12}{*}{\rotatebox{90}{\textbf{Qwen2.5-VL-3B-Instruct}}} & Dense & Acc. (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
%  & Dense & FLOPs (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
% \cline{2-13}
%  & FastV & Acc. (\% Dense) & -- & 97.6\% & 96.4\% & \textbf{100\%} & \textbf{99.9\%} & \textbf{97\%} & 98.9\% & \textbf{98.8\%} & 97.7\% & \textbf{98.3\%} \\
%  & FastV & FLOPs (\% Dense) & -- & 60.9\% & 63\% & 58\% & 63.9\% & 57.5\% & 54.8\% & 45.4\% & 57.7\% & 57.6\% \\
% \cline{2-13}
%  & PDrop & Acc. (\% Dense) & -- & 94.4\% & 91.8\% & 96.9\% & 97.8\% & 94.7\% & 95.4\% & 95.2\% & 93\% & 94.9\% \\
%  & PDrop & FLOPs (\% Dense) & -- & 56.1\% & 58.5\% & 52.8\% & 59.5\% & 52.3\% & \textbf{49.8\%} & 41.5\% & 52.9\% & 52.9\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 1\% & 100.3\% & \textbf{101\%} & 98.6\% & 86.9\% & 90.4\% & \textbf{99.3\%} & 97.5\% & \textbf{99.6\%} & 96.7\% \\
%  & P2P & FLOPs (\% Dense) & 1\% & 44.5\% & 45.1\% & 64.1\% & 36\% & 68.3\% & 96.9\% & 56.2\% & 65.6\% & 59.6\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 3\% & \textbf{100.3\%} & \textbf{101\%} & 98.1\% & 86.2\% & 86.1\% & 93.8\% & 91.9\% & 98.5\% & 94.5\% \\
%  & P2P & FLOPs (\% Dense) & 3\% & \textbf{40\%} & 45.1\% & 49.7\% & 31.9\% & 51.2\% & 82.5\% & 35.3\% & 56.4\% & 49\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 5\% & \textbf{100.3\%} & 99.1\% & 60.1\% & 85.4\% & 52.7\% & 23.6\% & 91.8\% & 95.1\% & 76\% \\
%  & P2P & FLOPs (\% Dense) & 5\% & \textbf{40\%} & \textbf{43\%} & \textbf{42.6\%} & \textbf{25.7\%} & \textbf{43.9\%} & 82.5\% & \textbf{33\%} & \textbf{49.6\%} & \textbf{45\%} \\
% \hline
% \multirow{12}{*}{\rotatebox{90}{\textbf{Qwen2.5-VL-7B-Instruct}}} & Dense & Acc. (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
%  & Dense & FLOPs (\% Dense) & -- & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
% \cline{2-13}
%  & FastV & Acc. (\% Dense) & -- & 82.6\% & 78.9\% & \textbf{98.3\%} & 94.7\% & \textbf{92.7\%} & 90.1\% & 98.3\% & 94.3\% & 91.3\% \\
%  & FastV & FLOPs (\% Dense) & -- & 61.8\% & 63.8\% & 58.9\% & 64.7\% & 58.5\% & 56.3\% & 47\% & 58.9\% & 58.7\% \\
% \cline{2-13}
%  & PDrop & Acc. (\% Dense) & -- & 79.8\% & 75.1\% & 92.9\% & 91.9\% & 89.7\% & 88.6\% & 93.6\% & 88.8\% & 87.5\% \\
%  & PDrop & FLOPs (\% Dense) & -- & 56.3\% & 58.7\% & 53\% & 59.7\% & 52.5\% & \textbf{50.4\%} & 42.3\% & 53.3\% & 53.3\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 1\% & \textbf{97.6\%} & \textbf{98.5\%} & -- & \textbf{97\%} & 87.7\% & \textbf{98.9\%} & \textbf{100.3\%} & \textbf{96.7\%} & \textbf{96.7\%} \\
%  & P2P & FLOPs (\% Dense) & 1\% & 48.1\% & 48\% & -- & 70.5\% & 46.2\% & 93.3\% & 72.5\% & 56.5\% & 62.2\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 3\% & 97.5\% & 94.2\% & 97.3\% & 96.8\% & 85.2\% & 89.1\% & 97.3\% & 93.9\% & 93.9\% \\
%  & P2P & FLOPs (\% Dense) & 3\% & 45.2\% & \textbf{39.9\%} & 44.1\% & 57.2\% & 43.1\% & 83.8\% & 47.8\% & 50.5\% & 51.4\% \\
% \cline{2-13}
%  & P2P & Acc. (\% Dense) & 5\% & 96.9\% & 94.2\% & 94.7\% & 92.2\% & 78.2\% & 88.9\% & 84.9\% & 86\% & 89.5\% \\
%  & P2P & FLOPs (\% Dense) & 5\% & \textbf{42.4\%} & \textbf{39.9\%} & \textbf{41\%} & \textbf{49.2\%} & \textbf{39.9\%} & 80.6\% & \textbf{29.3\%} & \textbf{41.5\%} & \textbf{45.5\%} \\
% \hline
% \end{tabular}
% \end{table*}
\begin{table}[t]
\centering
\caption{Overall accuracy and FLOPs relative to Dense, averaged over all available model--dataset pairs. Each pair is normalized to its corresponding Dense result before averaging. The best non-Dense accuracy and lowest non-Dense FLOPs are bolded.}
\label{tab:overall_baselines_p2p_average_percent_dense}

\begin{tabular}{llcc}
\hline
Method & Tol. & \begin{tabular}{@{}c@{}}Avg. Acc.\\(\% Dense)\end{tabular} & \begin{tabular}{@{}c@{}}Avg. FLOPs\\(\% Dense)\end{tabular} \\
\hline
Dense & -- & 100\% & 100\% \\
FastV & -- & 96.9\% & 55.3\% \\
PDrop & -- & 95.4\% & 50.2\% \\
P2P & 1\% & \textbf{97\%} & 58.5\% \\
P2P & 3\% & 94.1\% & 44.7\% \\
P2P & 5\% & 85.4\% & \textbf{38.5\%} \\
\hline
\end{tabular}
\end{table}
\begin{table}[t]
\centering
\caption{Average accuracy and inference latency percentages relative to Dense across all available combinations of the two LLaVA models and eight datasets. Each model--dataset pair is normalized by its own Dense result before averaging. Missing runs are ignored. The best non-Dense accuracy and lowest non-Dense latency are bolded.}
\label{tab:llava7b_13b_overall_percent_dense}

\begin{tabular}{llcc}
\hline
Method & Tol. & Avg. Acc. (\% Dense) & Avg. Latency (\% Dense) \\
\hline
Dense & -- & 100\% & 100\% \\
FastV & -- & 99\% & 99.9\% \\
PDrop & -- & \textbf{99.5\%} & 98.2\% \\
P2P & 1\% & 97.3\% & 84\% \\
P2P & 3\% & 94\% & \textbf{78.2\%} \\
P2P & 5\% & 88\% & 129.5\% \\
\hline
\end{tabular}
\end{table}

